CINS: Comprehensive Instruction for Few-shot Learning in Task-oriented Dialog Systems

As labeling cost for different modules in task-oriented dialog (ToD) systems is high, a major challenge in practice is to learn different tasks with the least amount of labeled data. Recently, prompting methods over pre-trained language models (PLMs) have shown promising results for few-shot learning in ToD. To better utilize the power of PLMs, this paper proposes Comprehensive Instruction (CINS) that exploits PLMs with extra task-specific instructions. We design a schema (definition, constraint, prompt) of instructions and their customized realizations for three important downstream tasks in ToD, i.e. intent classification, dialog state tracking, and natural language generation. A sequence-to-sequence model (T5) is adopted to solve these three tasks in a unified framework. Extensive experiments are conducted on these ToD tasks in realistic few-shot learning scenarios with small validation data. Empirical results demonstrate that the proposed CINS approach consistently improves techniques that finetune PLMs with raw input or short prompts.

==> tables/zero.tex <==
\begin{table}[t!]
    \centering
    \begin{tabular}{c|ccc}
        \toprule
           & \textbf{IC} & \textbf{DST} & \textbf{NLG}  \\
         \midrule
           STD & 0.0 & 0 & 16.0/15.8 \\
           PE &  0.0 & 0 &  6.4/10.8 \\
           \textsc{CIns} & 13.6 & 0 &  5.9/5.8 \\
        \bottomrule
    \end{tabular}
    \caption{Zero-shot results for different tasks in ToD. SER is reported for NLG. For NLG, we reported both SER and BLEU score seperated by `/'.}
    \label{table:zerp}
\end{table}
